LaPose: Laplacian Mixture Shape Modeling for RGB-Based Category-Level Object Pose Estimation

While RGBD-based methods for category-level object pose estimation hold promise, their reliance on depth data limits their applicability in diverse scenarios. In response, recent efforts have turned to RGB-based methods; however, they face significant challenges stemming from the absence of depth information. On one hand, the lack of depth exacerbates the difficulty in handling intra-class shape variation, resulting in increased uncertainty in shape predictions. On the other hand, RGB-only inputs introduce inherent scale ambiguity, rendering the estimation of object size and translation an ill-posed problem. To tackle these challenges, we propose LaPose, a novel framework that models the object shape as the Laplacian mixture model for Pose estimation. By representing each point as a probabilistic distribution, we explicitly quantify the shape uncertainty. LaPose leverages both a generalized 3D information stream and a specialized feature stream to independently predict the Laplacian distribution for each point, capturing different aspects of object geometry. These two distributions are then integrated as a Laplacian mixture model to establish the 2D-3D correspondences, which are utilized to solve the pose via the PnP module. In order to mitigate scale ambiguity, we introduce a scale-agnostic representation for object size and translation, enhancing training efficiency and overall robustness. Extensive experiments on the NOCS datasets validate the effectiveness of LaPose, yielding state-of-the-art performance in RGB-based category-level object pose estimation. Codes are released at https://github.com/lolrudy/LaPose

==> tables/Real_percat_abs.tex <==
\begin{table}[t]
    \centering
    \caption{Per-category results of LaPose (Ours) on NOCS-REAL275 using absolute evaluation metrics.}
    \label{tab:percat_realabs}
    \setlength{\tabcolsep}{1mm}
    \begin{tabular}{@{}c|c c c|c c c@{}}
    \toprule
        Category & $IoU_{25}$ & $IoU_{50}$ & $IoU_{75}$ & $5^\circ 5cm$ & $10^\circ 5cm$ & $10^\circ 10cm$ \\ \hline
        bottle & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 \\ 
        bowl & 47.8 & 24.8 & 8.9 & 24.8 & 27.8 & 52.6 \\
        camera & 44.6 & 12.0 & 0.1 & 0.3 & 5.4 & 15.3 \\ 
        can  & 33.2 & 11.7 & 1.6 & 7.7 & 26.9 & 63.9 \\ 
        laptop & 84.1 & 41.2 & 4.2 & 2.3 & 6.1 & 30.8 \\ 
        mug & 37.7 & 15.4 & 0.9 & 2.8 & 9.1 & 20.3 \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> tables/Real_percat_norm.tex <==
\begin{table}[t]
    \centering
    \caption{Per-category results of LaPose (Ours) on NOCS-REAL275 using scale-agnostic evaluation metrics.}
    \label{tab:percat_realnorm}
    \setlength{\tabcolsep}{1mm}
    \begin{tabular}{@{}c|c c c|c c c c c@{}}
    \toprule
        Category & $NIoU_{25}$ & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ & $0.2d$ & $0.5d$ & $10^\circ$ \\ \hline
        bottle & 41.1 & 16.3 & 1.2 & 16.7 & 45.5 & 18.6 & 50.4 & 51.1 \\ 
        bowl & 100.0 & 96.9 & 46.9 & 89.6 & 97.4 & 92.3 & 100.0 & 97.4 \\
        camera & 43.3 & 6.5 & 0.0 & 0.7 & 14.2 & 5.8 & 54.4 & 21.3 \\ 
        can  & 60.3 & 23.0 & 2.4 & 27.6 & 84.0 & 28.0 & 85.6 & 90.5 \\ 
        laptop & 80.3 & 71.6 & 27.0 & 52.4 & 60.0 & 63.1 & 83.6 & 60.6 \\ 
        mug & 96.4 & 73.1 & 17.0 & 37.6 & 43.1 & 73.4 & 98.9 & 43.2 \\ 
        \bottomrule
    \end{tabular}

\end{table}

==> tables/ablation_new.tex <==
\begin{table}[!t]
    \centering
    \caption{Ablation studies on NOCS-REAL275. $F_{conv}$ and $F_{dino}$ denote the semantic feature extracted by the convolutional network and DINOv2. 
    $\sigma^2$ denotes whether variances are predicted and fed into the PnP module.
    If $\sigma^2$ is used, the modeling distribution is either Gaussian (Gaus.) or Laplacian (Lap.).
    SAP denotes whether the scale-agnostic pose representation is used.
    % M.D. denotes that whether we estimate metric depth as in OLD-Net \cite{fan2022oldnet} or DINOv2 \cite{oquab2023dinov2} and use the Umeyama algorithm to solve the pose from the 3D-3D correspondences.
    }
    \label{tab:ablation}
    \tablestyle{5pt}{1.2}
    \begin{tabular}{@{}c|ccc|c|cc|cc@{}}
    \toprule
        No. & $F_{conv}$ & $F_{dino}$ & $\sigma^2$ & SAP  & $NIoU_{25}$ & $NIoU_{50}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ \\ \hline
        A & \checkmark & ~  & ~ & \checkmark  &  60.3 & 39.7 & 29.0 & 46.1 \\ 
        B & \checkmark & ~  & ~ & ~  & 37.8 & 17.6 & 10.5 & 33.2 \\ 
        % C & \checkmark & ~ & ~ & ~ & ~ & \cite{fan2022oldnet} & 29.7 & 5.1 & 1.7 & 13.5 \\ 
        % D & \checkmark & ~ & & ~ ~ & ~ & \cite{oquab2023dinov2} & 29.7 & 5.1 & 1.7 & 13.5 \\ 
        \hline
        C &  & \checkmark & ~  & \checkmark  & 61.7 & 26.9 & 16.9 & 38.5 \\ 
        D & \checkmark & \checkmark  &  & \checkmark & 64.9 & 42.1 & 32.5 & 52.8 \\
        \hline
        E & \checkmark &  & Lap.  & \checkmark  & 65.5 & 43.4 & 33.6 & 51.2 \\ 
        F & \checkmark &  & Gaus.  & \checkmark  & 59.1 & 37.6 & 28.3 & 44.7 \\ 
        \hline
        G &  & \checkmark & Lap.  & \checkmark  & 65.3 & 37.4 & 21.1 & 43.3 \\ 
        \hline
        H & \checkmark & \checkmark & Gaus.  & \checkmark  & 69.3 & 42.0 & 32.2 & 55.7 \\ 
        \hline
        I & \checkmark & \checkmark & Lap.  &  & 52.4 & 25.8 & 15.4 & 41.6 \\ 
        \hline
        J & \checkmark & \checkmark  & Lap. & \checkmark & \textbf{70.7} & \textbf{47.9} & \textbf{37.4} & \textbf{57.4} \\
\bottomrule
    \end{tabular}
    
\end{table}

==> tables/camera_abs_result.tex <==
\begin{table}[t]
    \centering
    \caption{Comparison with state-of-the-art methods on NOCS-CAMERA25 using evaluation metrics with absolute object scale.}
    \label{tab:camera_abs}
    \tablestyle{5pt}{1.2}
    \begin{tabular}{@{}c|c c c|c c c c c@{}}
    \toprule
        Method & $IoU_{25}$ & $IoU_{50}$ & $IoU_{75}$ & $10^\circ 10cm$ & $10cm$ \\ \hline
        MSOS \cite{lee2021msos} & 31.8 & 9.3 & 0.9 & 24.1 & 37.3   \\ 
        OLD-Net \cite{fan2022oldnet} & \textbf{36.4} & 10.3 & 0.6 & 26.7 & \textbf{40.8 } \\
        DMSR \cite{wei2023dmsr} & 35.4 & 11.2 & 1.3 & 33.0 & 39.3   \\ 
         \hline
        Ours & 33.3 & \textbf{11.4} & \textbf{1.6} & \textbf{34.1} & 38.6  \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> tables/camera_percat_abs.tex <==
\begin{table}[t]
    \centering
    \caption{Per-category results of LaPose (Ours) on NOCS-CAMERA25 using absolute evaluation metrics.}
    \label{tab:percat_synabs}
    \setlength{\tabcolsep}{1mm}
    \begin{tabular}{@{}c|c c c|c c c@{}}
    \toprule
        Category & $IoU_{25}$ & $IoU_{50}$ & $IoU_{75}$ & $5^\circ 5cm$ & $10^\circ 5cm$ & $10^\circ 10cm$ \\ \hline
        bottle & 37.3 & 11.8 & 1.7 & 6.2 & 7.5 & 27.6 \\ 
        bowl & 30.7 & 8.6 & 1.1 & 10.7 & 11.9 & 43.4 \\
        camera & 16.9 & 4.3 & 0.3 & 1.9 & 6.9 & 25.1 \\ 
        can  & 16.1 & 4.7 & 0.7 & 9.3 & 13.0 & 44.6 \\ 
        laptop & 70.7 & 31.3 & 5.2 & 4.5 & 9.7 & 31.2 \\ 
        mug & 27.7 & 7.5 & 0.6 & 4.7 & 9.3 & 32.5 \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> tables/camera_percat_norm.tex <==
\begin{table}[t]
    \centering
    \caption{Per-category results of LaPose (Ours) on NOCS-CAMERA25 using scale-agnostic evaluation metrics.}
    \label{tab:percat_synnorm}
    \setlength{\tabcolsep}{1mm}
    \begin{tabular}{@{}c|c c c|c c c c c@{}}
    \toprule
        Category & $NIoU_{25}$ & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ & $0.2d$ & $0.5d$ & $10^\circ$ \\ \hline
        bottle & 75.3 & 49.4 & 14.1 & 52.5 & 81.5 & 52.6 & 82.2 & 86.3 \\ 
        bowl & 94.0 & 77.4 & 22.9 & 72.8 & 94.7 & 73.2 & 95.2 & 95.9 \\
        camera & 65.1 & 29.3 & 2.9 & 18.8 & 56.0 & 25.7 & 77.1 & 66.0 \\ 
        can  & 74.3 & 42.6 & 8.5 & 31.9 & 76.9 & 31.9 & 77.0 & 85.6 \\ 
        laptop & 90.3 & 71.3 & 31.5 & 63.0 & 85.2 & 67.7 & 93.7 & 88.5 \\ 
        mug & 52.3 & 23.5 & 4.6 & 15.2 & 44.5 & 21.1 & 62.2 & 57.6 \\ 
        \bottomrule
    \end{tabular}

\end{table}
